Efficient OCR for Building a Diverse Digital History

Thousands of users consult digital archives daily, but the information they can access is unrepresentative of the diversity of documentary history. The sequence-to-sequence architecture typically used for optical character recognition (OCR) - which jointly learns a vision and language model - is poorly extensible to low-resource document collections, as learning a language-vision model requires extensive labeled sequences and compute. This study models OCR as a character level image retrieval problem, using a contrastively trained vision encoder. Because the model only learns characters' visual features, it is more sample efficient and extensible than existing architectures, enabling accurate OCR in settings where existing solutions fail. Crucially, the model opens new avenues for community engagement in making digital history more representative of documentary history.

==> figures/nara.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=.7\linewidth]{figs/NARA.png}
    \caption{\textbf{Diversity in the National Archives Dataset.} This figure shows examples sampled from the National Archives Zero-Shot evaluation dataset, along with EffOCR predicted transcriptions.} 
    \label{fig:nara}
    \vspace{-4mm}
  \end{figure*}

==> figures/network.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=.45\linewidth]{figs/network.png}
    \caption{\textbf{Supply Chain Networks (Japan, 1956).} Each node in the graph is a firm, whose size is proportional to its degree centrality in the supply chain network. Shading denotes three of the largest firms in pre-war Japan - Mitsui, Mitsubishi, and Sumitomo - as well as other firms - comprising Japan's largest conglomerates - targeted by the Holding Company Liquidation Commission (HCLC) in the late 1940s.}
    \label{fig:network}
    \vspace{-4mm}
  \end{figure}
  

==> tables/nara_zero_shot.tex <==
\begin{table}[ht]
    \centering
    \resizebox{.5\linewidth}{!}{
    \begin{threeparttable}
       \begin{tabular}{lcc}
    \toprule
OCR Model &	Character Error Rate	\\
\midrule
EffOCR-Word (Small)	& 0.126	\\
Tesseract OCR (Best) &	0.118	\\
EasyOCR	CRNN &	0.129	\\
PaddleOCR SVTR & 0.160	\\
Google Cloud Vision OCR	& 0.018 \\
TrOCR (Base) & 0.103 \\
TrOCR (Small) & 0.537 \\
    \bottomrule 
    \end{tabular}
    \end{threeparttable}}
    \caption{\textbf{Zero Shot Performance on National Archives Dataset.} This table reports off-the-shelf performance of different OCR architectures on a diverse dataset of US National Archives documents. }
        \label{comparisons_nara_table}
\end{table}

==> tables/poster_table.tex <==

       \begin{tabular}{lcccccccccccccc}
      \toprule
      &		&	&		& 	&	& \multicolumn{6}{c}{Character Error Rate} & &	\multicolumn{2}{c}{Lines/second} \\
	&		&	& 	&	&	&	Horiz.	&	Vertical 	&	Vertical	&	\multicolumn{2}{c}{Chron. Amer.}	& Anci. & &	Horiz. &	Chron. 	\\
Model/Engine	& Seq2Seq?	&	Transformer? & Pretraining	&	Parameters	& &	Jap.	&	Jap. (tables)	&	Jap. (prose)	&	Eval & Day/Decade	 & Greek & &	Jap.	&	Amer.	\\

\cmidrule{1-5} \cmidrule{7-12} \cmidrule{14-15} \\

EffOCR-C (Base)	&	$\times$ & $\times$ 	&	from scratch	&	112.5 M	&&	\underline{\textbf{0.006}}	&	\underline{\textbf{0.007}}	& 0.030 & 0.023 & 0.062 & 0.049  & & 0.79 & 0.49	\\ \\

EffOCR-C (Small)	&	$\times$ & $\times$ 	&	from scratch	&	9.3 M	&	& 0.010 & 0.009 & 0.036 & 0.028 & 0.080 & 0.052 && 19.46 & 13.40	\\ \\
EffOCR-T (Base) & $\times$ & $\checkmark$ & from scratch & 101.8 M&& 0.009 & 0.007 & \underline{\textbf{0.027}} & 0.022 & 0.059 & \underline{\textbf{0.047}} & & 0.19 & 0.31 \\ \\

EffOCR-Word (Small) &	$\times$ & $\times$ 	&	from scratch	&	10.6 M	&	& - & - & - & 0.015 & 0.043 & - && - & 21.36	\\ \\
 \\

Google Cloud Vision OCR &  ? & ?	&	off-the-shelf	&	?	& &	0.173	&	0.695	&	0.135	&	\underline{\textbf{0.005}} & \underline{\textbf{0.019}} & 0.065 & & ? & ?	\\ \\

Baidu OCR	&	? & ?	&	off-the-shelf	&	? 	& &	0.060	&	0.556	&	0.177	& -&	- & - & & ? & ?	\\ \\

Tesseract OCR (Best) 	&	$\checkmark$ & $\times$	&	off-the-shelf	& 1.4 M & &	1.021	&	0.996	&	0.744	&	0.106 & 0.170  & 0.251 & & 4.90 & 4.47	\\ \\

EasyOCR CRNN 	& $\checkmark$	&	$\times$ &	off-the-shelf	&	3.8 M	&&	0.191	&	- 	&	 -	&	0.170 & 0.274  & - & & 33.55 & 19.80 	\\
	&	&	&	fine-tuned	&		&	 &	0.082	&	 -	&	 -	&	0.036 & 0.157	\\
 
     &    &    & from scratch & 	&	&	0.132	&	 -	&	 -	&	0.131  & 0.204 &  \\ \\
   
PaddleOCR SVTR	&  $\times$	& $\times$	&	off-the-shelf	&	11 M	& &	0.085	&	 -	&	 -	&	0.304 & 0.314 & - & & 13.34 & 13.56	\\
	&	&	&	fine-tuned	&		&&	0.032	&	 -	&	- 	&	0.103 & 0.129 & \\
     &   & & from scratch &		&	&	0.097	&	- 	&	- 	&	0.104 &	0.138 & \\ \\
  
TrOCR (Base)	& $\checkmark$	& $\checkmark$ &	off-the-shelf	&	334 M	&		&	-	&	-	&	-	&	0.015 & 0.038 & - & & - & 0.43	\\
&	&		&	fine-tuned	&				&& -	&	-	&	-	&	0.013 & 0.027	\\
    &    & & from scratch &		&		&	-	&-	&	-	&	0.809 & 0.831 &	 \\ \\
 
TrOCR (Small)	& $\checkmark$  &	$\checkmark$ 	&	off-the-shelf	&	62 M	&&	- &	-	&	-	&	0.039 & 0.121 & - & & - & 0.97	\\
	&	&	&	fine-tuned	&		&		& -	&	-	&	-	&	0.075 & 0.091 &	\\
      &  & & from scratch &		&		& - &	-	&	-	&	0.773 & 0.820 &	 \\
 
    \bottomrule 
    \end{tabular}



